Direct Preference-Based Evolutionary Multi-Objective Optimization with Dueling Bandit

Optimization problems find widespread use in both single-objective and multi-objective scenarios. In practical applications, users aspire for solutions that converge to the region of interest (ROI) along the Pareto front (PF). While the conventional approach involves approximating a fitness function or an objective function to reflect user preferences, this paper explores an alternative avenue. Specifically, we aim to discover a method that sidesteps the need for calculating the fitness function, relying solely on human feedback. Our proposed approach entails conducting direct preference learning facilitated by an active dueling bandit algorithm. The experimental phase is structured into three sessions. Firstly, we assess the performance of our active dueling bandit algorithm. Secondly, we implement our proposed method within the context of Multi-objective Evolutionary Algorithms (MOEAs). Finally, we deploy our method in a practical problem, specifically in protein structure prediction (PSP). This research presents a novel interactive preference-based MOEA framework that not only addresses the limitations of traditional techniques but also unveils new possibilities for optimization problems.

==> makefile <==
FILE=main

all:	
	latex $(FILE)
	bibtex $(FILE)
	latex $(FILE)
	latex $(FILE)
	dvips -o $(FILE).ps $(FILE).dvi
	ps2pdf $(FILE).ps
	open $(FILE).pdf

clean:
	rm -f *.aux *.blg *.log *.bbl *.out *.bak *.synctex.gz *.synctex.gz\(busy\) *.tex~

cleanall: clean
	rm -f *.dvi $(FILE).ps $(FILE).pdf


==> related_work.tex <==
%!TeX root=main.tex

\section{Related Work}
\label{sec:related}

\subsection{Multi-objective decision making}
\begin{itemize}
    \item RLHF
    \item MOMAB
\end{itemize}
\subsection{Consultation methods}
\begin{itemize}
    \item fitness function based: PBO, RL with reward
    \item solution based: bandit, dueling bandit, high-dimensional (clustering multi-armed, independent bandits).
\end{itemize}





% \subsection{Single-objective Problem}

% \subsection{Multi-objective Problem}
% \color{red}
% \subsection{Preference Learning}
% % \color{red}
% % classification: priori, posterior, interactive
% % \color{black}

% Preference learning can be divided into three categories: priori, posteriori and interactive based on the timing of consultation. Interactive preference elicitation~\cite{LiLDMY20} presents a valuable opportunity for the DM to gradually comprehend the underlying black-box system and consequently refine user preference information.

% Preference learning has received significant attention in research. The process of preference learning can be categorized into two types: fitness-function based or fitness-function free. 
% The first type, which is widely explored~\cite{JacquetS82,Furkranz03,ChuG05,HoulsbyHFL11,HoulsbyHHG12,ZintgrafRLJN18}, involves approximating a value function that represents user preference using mathematical tools such as Gaussian process (GP), neural network (NN) and others. Fitness-based method can be traced back to 1982. ~\cite{JacquetS82} introduced the UTA (UTilités Additives) method for deducing value functions based on a provided ranking of reference set. 
% % In 2003,~\cite{Furkranz03} employed pairwise preference to predict a ranking, representing a total order, for potential labels associated with new training examples. 
% In 2005,~\cite{ChuG05} utilized GP for pairwise preference learning (PGP) within a Bayesian framework. 
% % In 2007,~\cite{CaoQLML07} proposed ListNet, a NN-based learning-to-rank method. In 2011,~\cite{HoulsbyHFL11} used GP classification integrated with information theory to select the best solution with maximum entropy. In 2012,~\cite{HoulsbyHHG12} extended their work to handle multi-user scenarios by introducing weight vector for each user and combining multiple preference latent functions. 
% A study conducted in 2018~\cite{ZintgrafRLJN18} compared four prominent preference elicitation modules and found that ranking queries outperformed the pairwise and clustering approaches in terms of utility models ad human preference. 
% However, recent studies have explored an alternative method of preference learning that do not involve approximating value functions. This approach is inspired by ~\cite{YanLCCVC22} in 2022 who proposed a novel method for conducting pairwise preference judgments using double Thompson sampling (DTS) approach~\cite{WuL16}. Similar idea have also emerged in the realm of RL preference learning~\cite{MyersBS23active}.


% \subsection{Preference-based active learning} 

% Preference-based active learning has been considered in the study by~\cite{MyersBS23active} and has been utilized in various fields such as classification tasks~\cite{ChenBCH13,ChenHK17} and ranking aggregation~\cite{ChenBCH13}. However none of these approaches address our specific problem of adaptively requesting pairwise comparisons between solutions in an online setting for PL.
% % ~\cite{MyersBS23active} also considers preference-based active learning~\cite{Settles09,RenXCHLGCW21,KumarG20}.  Outside RL, preference-based active learning has been used for classification tasks~\cite{ChenBCH13,ChenHK17} and ranking aggregation~\cite{ChenBCH13}. None of these approaches have tackled our problem of adaptively asking for pairwise comparisons between solutions at deployment to conduct preference learning in an online setting.

% As mentioned earlier~\cite{YanLCCVC22}, the dueling bandit algorithm shows promise as a solution that does not involve the direct calculation of the value function. However, there is currently no dueling bandit algorithm designed specifically for active learning~\cite{Settles09,RenXCHLGCW21,KumarG20}. The state-of-art active bandit algorithms have predominantly been developed for multi-armed bandit (MAB) problems~\cite{BaramYL04,AntosGS08,CarpentierLGNA11,GantiG12,GantiG13,GlimsdalG19,ZhangJJ20}.
% %~\cite{BaramYL04} considered each arm as an active learner and proposed a method that used EXP3 and EXP4 to recommend the appropriate active algorithm for different scenarios.~\cite{AntosGS08} introduced GAFS-MAX, which selected under-sampled points or arms with maximum loss, and redefined the regret equation based on the loss function in active learning.~\cite{CarpentierLGNA11}, using the same regret definition as ~\cite{AntosGS08}, constructed the upper confidence bound (UCB) function in two forms with the Chernoff-Heoffding and Bernstein allocation strategies respectively. Inspired by previous work~\cite{GantiG12},~\cite{GantiG13} proposed LCB-AL which aimed to minimize the uncertainty level measured by lower confidence bound (LCB).


% \subsection{Dueling Bandit}
% %To address the problem of adaptively collecting pairwise comparisons between solutions in an online setting for preference learning, we propose an active dueling bandit algorithm. This algorithm not only actively selects solutions to be queried but also performs preference learning using pairwise comparisons, similar to the dueling bandit framework. 

% The dueling bandits problem involves a sequential decision-making process where a learner selects two out of $K$ “arms” in each round and receives real-valued feedback. As described in~\cite{BengsBEH21}, dueling bandits can be grouped into 3 categories: MAB-related, merge sort/quick sort, and tournament/challenge. In this paper, our focus is on traditional dueling bandits, specifically those that fall within the MAB-related categorized. 

% Among the traditional dueling bandit algorithms, there are four distinct methods for making pairwise comparisons:  explore then commit (ETC) (e.g., interleaved filtering (IF)~\cite{YueBKJ12}, beat the mean (BTM)~\cite{YueJ11} and SAVAGE~\cite{UrvoyCFN13}), upper confidence bound (UCB) (e.g., relative upper confidence bound (RUCB)~\cite{ZoghiWM14}, MergeRUCB~\cite{ZoghiWR15}, and relative confidence sampling (RCS)~\cite{ZoghiWDM14}), Thompson sampling (e.g., double Thompson sampling (DTS)~\cite{WuL16} and MergeDTS~\cite{LiMRZ20}), and minimum empirical divergence (e.g., relative minimum empirical divergence (RMED)~\cite{KomiyamaHKN15} and deterministic minimum empirical divergence (DMED)~\cite{HondaT10}).
% %The first method is known as explore then commit (ETC), which is utilized by algorithms such as interleaved filtering (IF)~\cite{YueBKJ12},  beat the mean (BTM)~\cite{YueJ11} and SAVAGE~\cite{UrvoyCFN13}. ETC methods kick out solutions that are unlikely to win, but this approach may lead to lower predictive probability accuracy. The second method involves using the upper confidence bound (UCB), for example relative upper confidence bound (RUCB)~\cite{ZoghiWM14}, MergeRUCB~\cite{ZoghiWR15}, and relative confidence sampling (RCS)~\cite{ZoghiWDM14}. MergeRUCB, an extension of RUCB, is particularly designed for scenarios with a large number of arms. RCS combines UCB and Beta posterior distribution to recommend one arm for each duel in each iteration step. The third method employs Thompson sampling, as demonstrated by double Thompson sampling (DTS)~\cite{WuL16} and MergeDTS~\cite{LiMRZ20}. Similar to MergeRUCB, MergeDTS is designed for dealing with a substantial number of arms. It is worth nothing that UCB methods assume the existence of a Condorcet winner, whereas Thompson sampling methods assume a Copeland winner, representing a fundamental distinction between these two types. The fourth method involves using the minimum empirical divergence, as introduced by relative minimum empirical divergence (RMED)~\cite{KomiyamaHKN15} and deterministic minimum empirical divergence (DMED)~\cite{HondaT10}. RMED and DMED employee KL divergence as a metric to evaluate candidate arms. Overall, these four methods represent different approaches to pairwise comparison in traditional dueling bandit algorithms.
% In this paper, our proposed method is inspired by RUCB. We build upon the assumption of the existence of a Copeland winner, strengthening the reliability of our proposed method. Additionally, similar to RUCB, our method incorporates the confidence level into the decision-making process. This feature allows us to provide a recommendation confidence.

% % \begin{itemize}
% %     \item In~\cite{ZoghiWM14}, RUCB outperforms BTM and Condorcet SAVAGE with respect to regret and accuracy. And BTM and Condorcet SAVAGE were shown to outperform IF~\cite{YueJ11,UrvoyCFN13}.
% %     \item Apart from avoiding the burden of computing fitness function, we also want to give a confidence level of our recommended point $W^*$. Choosing RUCB as our baseline algorithm can help us utilize the confidence information in the preference learning process.
% % \end{itemize}

% % \subsection{Active Learning}

% % The purpose of active learning~\cite{Settles09,RenXCHLGCW21,KumarG20} is to query the least number of solutions to get the most accurate classification results. For our case, we would like active learning to alleviate information gain in each comparison and reduce total query times. There are many active MAB algorithms up to now~\cite{BaramYL04,AntosGS08,CarpentierLGNA11,GantiG12,GantiG13,GlimsdalG19,ZhangJJ20}.~\cite{BaramYL04} takes every arm as an active learner. By using EXP3 and EXP4, their proposed method is able to recommend a proper active algorithm for different scenarios.~\cite{AntosGS08} proposed GAFS-MAX selecting arms that are assumed as under-sampled points or have a maximum loss. Also they rewrite the regret equation according to the loss function in active learning.~\cite{CarpentierLGNA11} based on the same regret definition as ~\cite{AntosGS08} build the UCB function in two forms with the Chernoff-Heoffding and Bernstein allocation strategies respectively.  Inspired by previous work~\cite{GantiG12},~\cite{GantiG13} proposed LCB-AL which has an optimization target of minimizing the uncertainty level measured by LCB. 

% \color{black}


==> settings.tex <==
%!TeX root=main.tex

\section{Experimental Settings}
\label{sec:experiment_setting}

This section outlines some key experimental setup including benchmark test problems and performance metrics. More detailed information can be found in~\pref{app:experimental_setup}.

\paragraph{Benchmark problems}

In our experiments, we consider $33$ \textit{synthetic test instances} including ZDT1 to ZDT4 and ZDT6 ($m=2$) from ZDT~\cite{ZitzlerDT00}, DTLZ1 to DTLZ6 in DTLZ where $m=\{3,5,8,10\}$~\cite{DebTLZ05}, and WFG1, WFG3, WFG5, and WFG7 ($m=3$) from WFG~\cite{HubandHBW06}. These problems are with various PF shapes and different difficulties such as bias, plateau, and multi-modal. In addition, we also consider two \textit{scientific discovery problems} including a $4$-objective protein structure prediction (PSP) task~\cite{ZhangGLXC23} and a $2$-objective RNA inverse design problem~\cite{??}. The problem formulations are detailed in~\cref{app:real-world problems}.

%\subsection{Peer algorithms}
%\label{sec:peers}
%
%Our proposed algorithms are compared against two types of peer algorithms.
%\begin{itemize}
%    \item The first one is selected from three state-of-the-art PBEMO algorithms including \texttt{I-MOEAD-PLVF}~\cite{LiCSY19}, \texttt{I-NSGA2/LTR}~\cite{LiLY23}, \texttt{IEMO/D}~\cite{TomczykK19}.
%
%    \item The second type of algorithms are used in our ablation study. Specifically, to validate the effectiveness of our proposed stochastic dueling bandit algorithm, we replace it with the double Thompson sampling (DTS) used in conventional stochastic dueling bandits~\cite{WuL16} and preference learning algorithm in continuous space from Bayesian optimization~\cite{GonzalezDDL17}, respectively, in the \texttt{consultation} module. They are denoted as \our\texttt{-DTS} and \our\texttt{-PBO}, respectively. The step-by-step algorithmic implementation can be found in~\cref{app:step}. Parameter settings are given in~\cref{app:parameters}.
%\end{itemize}

%In ablation experiment, we design two algorithms. This first is to use DTS as consultation module and NSGA-II as optimization module. Additionally, PBO~\cite{GonzalezDDL17}, the pairwise preference learning method using Bayesian optimization module, is also implemented in our DPBEMO framework, acting as the consultation module. The step-by-step processes of the $2$ algorithms for ablation experiment can be referenced in~\cref{app:step}.

% \subsection{Parameter settings}
% \label{sec:parameter_settings}

% While the winning probability is usually known a priori in dueling bandits, it however does not exist in the context of MO. In this paper, to project a MO solution to an arm in the bandit setting, we define the winning probability $p_{i,j}$ of a pair of candidate solutions $\langle\mathbf{x}_i,\mathbf{x}_j\rangle,\forall i,j\in\{1,\ldots,N\}$ as~\cite{DingZ18}:
% \begin{equation}
%     p_{i,j}=\mu(V(\mathbf{x}_i)-V(\mathbf{x}_j)),
%     \label{eq:pij}
% \end{equation}
% where $\mu(a)=1/(1+\exp(-a))$, $V$ denotes the real preference distribution of each arm. Note that $p_{i,j}$ can take other forms in case it satisfies the conditions in~\pref{def:mab}. The other algorithmic parameters used in our experiments can be found in~\cref{app:parameters}.

\subsection{Performance metrics}
\label{sec:metrics}

As discussed in~\cite{LiDY18}, quality assessment of non-dominated solutions is far from trivial when considering DM's preference information regarding conflicting objective. In our experiments, we consider the following two metrics to serve this purpose.
\begin{itemize}
    \item The first one is the \textit{approximation accuracy} that evaluates the closeness of the best non-dominated solution to the DM preferred one:
        \begin{equation}
            \epsilon^\star(\mathcal{S})=\min_{\mathbf{x}\in\mathcal{S}}\|\mathbf{x}-\mathbf{x}^\star\|_2,
        \end{equation}
        where $\|\cdot\|_2$ is the Euclidean norm, $\mathbf{x}^\star$ is the \lq golden solution\rq\ specified by the DM but is unknown to the algorithm, and $\mathcal{S}$ is the non-dominated solutions set obtained by PBEMO.

    \item The second one is the \textit{average accuracy} that evaluates the average distance of all non-dominated policies in $\Pi$ to the DM preferred one:
        \begin{equation}
            \bar{\epsilon}(\mathcal{S})=\frac{\sum_{\mathbf{x}\in\mathcal{S}}\|\mathbf{x}-\mathbf{x}^\star\|_2}{|\mathcal{S}|},
        \end{equation}
        where $|\cdot|$ is the cardinality of a set.
\end{itemize}
The settings of $\mathbf{x}^\star$ used in our experiments are in~\cref{app:parameters}. Due to the stochastic nature of evolutionary computation, each experiment is repeated $20$ times with different random seeds. 
%We apply the widely used Wilcoxon signed-rank test~\cite{Wilcoxon92}, a non-parametric pairwise statistical test, to assess the statistical significance of our findings. In particular, the significance level is set to $p=0.05$ in our experiments.

%In our experiments, we consider two types of metrics. The first one is the approximation error regarding the ground truth 
%\begin{equation}
%    Loss=\min_{i\in\{1,2,\ldots,N\}}dist(\mathbf{z}_i,\mathbf{z}^r),
%    \label{eq:min_dis}
%\end{equation}
%where $\mathbf{z}^r$ denotes the global optima that user prefers most, $dist(\mathbf{z,z}^r)$ is the Euclidean distance between $\mathbf{z}^r$ and a solution $\mathbf{z}_i$ in the objective space.
 
% The \texttt{D-PBEMO} framework for three different optimization methods are specifically designed to address high-dimensional MOPs. To avoid excessive dispersion of the large-scale population, which can lead to a dilemma, an interactive EMO algorithm should not only seek solutions that best align with the user preferences but also aim to bring the entire population of candidate solutions as close as possible to the DM's ROI. Ensuring that the range of distribution of all candidate solutions within the population is as small as possible near the DM's preferred points is more advantageous. This concentrated distribution facilitates the DM in selecting the most suitable solution from a group of mutually non-dominated candidate solutions as the ultimate decision plan. 

%Additionally, to explore the degree of dispersion in the final populations obtained by different algorithms and to quantitatively measure the overall quality of all candidate solutions in the population, the following evaluative criterion for candidate solutions in MOPs with preferences is defined:
%\begin{equation}
%    \overline{Loss}={1\over N}\sum_{i\in\{1,2,\ldots,N\}} dist(\mathbf{z}_i,\mathbf{z}^r).
%\end{equation}

%To offer a statistical interpretation of the significance of comparison results, we conduct each synthetic problems 20 times. To analyze the data, we employ the Wilcoxon signed-rank test~\cite{Wilcoxon92} in our empirical study.

%The Wilcoxon signed-rank test, a non-parametric statistical test, is utilized to assess the significance of our findings. The test is advantageous as it makes minimal assumptions about the data's underlying distribution. It has been widely recommended in empirical studies within the EA community~\cite{DerracGMH11}. In our experiment, we have set the significance level to $p=0.05$.


%\subsection{Research Questions}
%
%In this paper, we mainly focus on the following 3 research questions (RQs):
%\begin{itemize}
%    % \item \textit{\underline{RQ1}}: What is the performance of our D-PBEMO algorithms on synthetic problems?
%    \item \textit{\underline{RQ1}}: What is the performance of our proposed method on traditional test problem suite comparing to peer algorithms?
%    \item \textit{\underline{RQ2}}: Whether our proposed method still works well on the practical problem, PSP?
%    \item \textit{\underline{RQ3}}: Whether our proposed method still works well on the robot control problem?
%
%\end{itemize}
% The performance metrics are listed in~\cref{app:performance_metric}.
% Note that the smaller the value of $dist(\mathbf{z,z}^r)$, the better.

